Communication Efficient Checking of Big Data Operations

We propose fast probabilistic algorithms with low (i.e., sublinear in the input size) communication volume to check the correctness of operations in Big Data processing frameworks and distributed databases. Our checkers cover many of the commonly used operations, including sum, average, median, and minimum aggregation, as well as sorting, union, merge, and zip. An experimental evaluation of our implementation in Thrill (Bingmann et al., 2016) confirms the low overhead and high failure detection rate predicted by theoretical analysis.

==> makros2.tex <==
% Macropackage of Peter Sanders
% =============================
%
% SE, 07.01.99: \prob, \expect, \var modified
% SE, 26.01.99: joined with macros of SE

\usepackage{color}
% allgemeine mathematische Notation
%\newcommand{\Id}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\seq}[1]{\left\langle #1\right\rangle}
\newcommand{\seqGilt}[2]{\left\langle #1\gilt #2\right\rangle}
\newcommand{\Id}[1]{\ensuremath{\textsf{#1}}}
\newcommand{\ceil}[1]{\left\lceil #1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\enorm}[1]{\norm{#1}_{2}}
\newcommand{\sumnorm}[1]{\norm{#1}_{1}}
\newcommand{\maxnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\xor}{\oplus}
\newcommand{\set}[1]{\left\{ #1\right\}}
\newcommand{\gilt}{:}
%\newcommand{\sodass}{\,:\,}
\newcommand{\sodass}{\mid}
\newcommand{\setGilt}[2]{\left\{ #1\gilt #2\right\}}
\newcommand{\Def}{:=}
\newcommand{\zvektor}[2]{\left(#1,#2\right)}
\newcommand{\vektor}[2]{\left(\begin{smallmatrix}#1\\#2\end{smallmatrix}\right)}
\newcommand{\condition}[1]{\left[#1\right]}
\newcommand{\binomial}[2]{\binom{#1}{#2}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\mymod}{\,\bmod\,}
\newcommand{\card}[1]{\left\vert{#1}\right\vert}
% \newcommand{\divides}{|}

\newcommand{\ld}{\mathrm{log}\,}
% Typen
\newcommand{\nat}{\mathbb{N}}
\newcommand{\natnull}{\mathbb{N}_{0}}
%\newcommand{\natless}[1]{\mathbb{N}_{<#1}}
\newcommand{\natless}[1]{\mathbb{N}_{#1}}
\newcommand{\nplus}{\mathbb{N}_+}
\newcommand{\real}{\mathbb{R}}
\newcommand{\rplus}{\mathbb{R}_+}
\newcommand{\rnneg}{\mathbb{R}_{\geq 0}}
\newcommand{\integer}{\mathbb{Z}}
% \newcommand{\intint}[2]{\set{#1,\ldots, #2}}
\newcommand{\intint}[2]{{#1}..{#2}}
\newcommand{\realrange}[2]{\left[#1, #2\right]}
\newcommand{\realrangeo}[2]{\left(#1, #2\right)}
\newcommand{\realrangelo}[2]{\left(#1, #2\right]}
\newcommand{\realrangero}[2]{\left[#1, #2\right)}
\newcommand{\unitrange}[2]{\realrange{0}{1}}
\newcommand{\bool}{\set{0,1}}
%\newcommand{\boolean}{\mathbb{B}}
%\newcommand{\mapping}[2]{#1\rightarrow #2}
\newcommand{\mapping}[2]{{#2}^{#1}}
\newcommand{\powerset}[1]{{\cal P}\left(#1\right)}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\Bild}{\mathbf{Bild}\:}

% Typannotation
\newcommand{\withtype}[1]{\in#1}

% Wahrscheinlichkeitsrechnung
\newcommand{\prob}[1]{{\mathbf{P}}\left[#1\right]}
\newcommand{\condprob}[2]{{\mathbf{P}}\left[#1\;|\;#2\right]}
\newcommand{\condexpect}[2]{{\mathbf{E}}\left[#1\;|\;#2\right]}
\newcommand{\expect}[1]{{\mathbf{E}}\left[#1\right]}
\newcommand{\var}{{\mathbf{V}}}
\newcommand{\quant}[2]{\tilde{#1}_{#2}}

% asymptotische Notation
\newcommand{\whpO}[1]{\tilde{\mathrm{O}}\left( #1\right)}
\newcommand{\Oschlange}{$\tilde{\mathrm{O}}$}
\newcommand{\Ohh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\Oh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\Ohlarge}[1]{\mathcal{O}\!\left( #1\right)}
% \newcommand{\Oh}[1]{{\mathcal{O}}(#1)}
\newcommand{\Ohsmall}[1]{\mathcal{O}(#1)}
\newcommand{\oh}[1]{\mathrm{o}\!\left( #1\right)}
\newcommand{\Th}[1]{\Theta\!\left( #1\right)}
\newcommand{\Thsmall}[1]{\Theta(#1)}
\newcommand{\Om}[1]{\Omega\left(#1\right)}
\newcommand{\Omsmall}[1]{\Omega(#1)}
\newcommand{\om}[1]{\omega\!\left( #1\right)}
\newcommand{\Oleq}{\preceq}

% local reference
\newcommand{\lref}[1]{\ref{\labelprefix:#1}}
\newcommand{\llabel}[1]{\label{\labelprefix:#1}}
\newcommand{\labelprefix}{} % later redefined using renewcommand

% Diskussion
\newcommand{\discussionsize}{\small}
\newenvironment{discussion}{\par\discussionsize}{\par}

% open issues
%\newcommand{\frage}[1]{\makebox[0cm]{$\bigotimes$}\marginpar{\tiny #1}}
\newcommand{\frage}[2][?]{\impmark{#1}{[\textcolor{red}{\textbf{#2}}]}}
\newcommand{\psfrage}[2][?]{\impmark{ps#1}{[\textcolor{blue}{\textbf{#2}}]}}

\usepackage{xparse}
\NewDocumentCommand\todo{G{*}}{\frage[TODO]{#1}}

\usepackage{xifthen}
\usepackage[normalem]{ulem}
\newcommand{\impmark}[1]{\strut\vadjust{\domark{#1}}}
\newcommand{\domark}[1]{\vbox to 0pt{\kern-\dp\strutbox\smash{\llap{\textbf{\textcolor{red}{#1}}\kern1em}}\vss}}
\makeatletter
\font\uwavefont=lasyb10 scaled 652
\def\dodgyText{\bgroup \markoverwith{\lower3.5\p@\hbox{\uwavefont \textcolor{red}{\char58}}}\ULon}
\makeatother
\newcommand{\dodgy}[2][]{\impmark{\ifthenelse{\isempty{#1}}{***}{* #1}}\dodgyText{#2}}

\newcommand{\mysubsubsection}[1]{\vspace{2mm}\noindent{\bf #1 }}
\newcommand{\fakesubsub}[1]{\par\medskip\noindent\textbf{#1 }}

\newenvironment{repeatThm}[1]{\par\medskip\noindent\textbf{#1.}\it}{}

% punkt am ende von display math
\newcommand{\punkt}{\enspace .}

% Pseudocode Unterst\"utzung
\newenvironment{code}{\noindent\normalsize%\sf%
\begin{tabbing}%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\kill}{\end{tabbing}}

% 1=pos, 2=llable, 3=caption
\newcommand{\labelcommand}{}
\newcommand{\captiontext}{}
\newsavebox{\codeparam}
\newcounter{lineNumber}
\newenvironment{disscodepos}[3]{%
\renewcommand{\labelcommand}{#2}%
\renewcommand{\captiontext}{#3}%
\sbox{\codeparam}{\parbox{\textwidth}{#3}}%
\begin{figure}[#1]\begin{center}\begin{code}\setcounter{lineNumber}{1}}{%
\end{code}\end{center}\caption{\llabel{\labelcommand}\captiontext}\end{figure}}

\newenvironment{disscode}[2]{\begin{disscodepos}{htb}{#1}{#2}}%
{\end{disscodepos}}

% code in text
%\newcommand{\codel}[1]{\textsf{#1}}
%\newcommand{\codem}[1]{\mathsf{#1}}
\newcommand{\codel}[1]{\mbox{\rm "`#1"'}}
\newcommand{\codem}[1]{\mathrm{#1}}
\newcommand{\Of}{\ensuremath{\textbf{of\ }}}
\newcommand{\Declare}[2]{#1\mbox{ \rm : }#2}
\newcommand{\DeclareInit}[3]{#1 = #3 \mbox{ \rm : }#2}

\newcommand{\Assert}{\textbf{Assert\ }}
\newcommand{\id}{\tt}
\newcommand{\Function} {\textbf{Function\ }}
\newcommand{\Funct}[3]{\Function #1\Declare{{\rm (}{#2\rm )}}{#3}}
\newcommand{\Procedure}{\textbf{Procedure\ }}
\newcommand{\Process}{\textbf{process\ }}
\newcommand{\While}    {\textbf{while\ }}
\newcommand{\Repeat}   {\textbf{repeat\ }}
\newcommand{\Until}    {\textbf{until\ }}
\newcommand{\Loop}     {\textbf{loop\ }}
\newcommand{\Exit}     {\textbf{exit\ }}
\newcommand{\Goto}     {\textbf{goto\ }}
\newcommand{\Do}       {\textbf{do\ }}
\newcommand{\Od}       {\textbf{od\ }}
\newcommand{\Dopar}       {\textbf{dopar\ }}
\newcommand{\For}      {\textbf{for\ }}
\newcommand{\Foreach}      {\textbf{foreach\ }}
\newcommand{\Is}{\mbox{\rm := }}
\newcommand{\Rof}      {\textbf{rof\ }}
\newcommand{\Forall}      {\textbf{forall\ }}
\newcommand{\To}       {\textbf{to\ }}
\newcommand{\Downto}       {\textbf{to\ }}
\newcommand{\If}       {\textbf{if\ }}
\newcommand{\Endif}    {\textbf{endif\ }}
\newcommand{\Fi}       {\textbf{fi\ }}
\newcommand{\Then}     {\textbf{then\ }}
\newcommand{\Else}     {\textbf{else\ }}
\newcommand{\Elsif}    {\textbf{elsif\ }}
\newcommand{\Return}   {\textbf{return\ }}
\newcommand{\Set}      {\textbf{set\ }}
\newcommand{\Boolean}  {\textbf{boolean\ }}
\newcommand{\Integer}  {$\integer$}
\newcommand{\True}     {\textbf{true\ }}
\newcommand{\False}    {\textbf{false\ }}
\newcommand{\Bitand}   {\textbf{bitand\ }}
\newcommand{\Var}      {\textbf{var\ }}
\newcommand{\Xor}       {\textbf{\ xor\ }}
\newcommand{\Not}       {\textbf{\ not\ }}
\newcommand{\Or}       {\textbf{\ or\ }}
\newcommand{\Div}       {\textbf{\ div\ }}
\newcommand{\Mod}       {\textbf{\ mod\ }}
\newcommand{\ForFromToPar}[3]{{\For $#1 \Is #2$ \To $#3$ \Dopar}}
\newcommand{\ForFromTo}[3]{{\For $#1$ \Is $#2$ \To $#3$ \Do}}
\newcommand{\ForFromDownto}[3]{{\For $#1$ \Is $#2$ \Downto $#3$ \Do}}
\newcommand{\ForFromWhile}[3]{{\For $#1$ \Is $#2$ \To $\infty$ \While $#3$ \Do}}
\newcommand{\ForFromdownWhile}[3]{{\For $#1$ \Is $#2$ \Downto $-\infty$ \While $#3$ \Do}}
\newcommand{\ForFromToStep}[4]{{\For $#1$ \Is $#2$ \To $#3$ \Step $#4$  \Do}}
\newcommand{\ForFromDowntoStep}[4]{{\For $#1$ \Is $#2$ \Downto $#3$  \Step $#4$ \Do}}
\newcommand{\ForFromStepWhile}[4]{{\For $#1$ \Is $#2$ \To $\infty$ \Step $#3$  \While $#4$ \Do}}
\newcommand{\ForFromdownStepWhile}[4]{{\For $#1$ \Is $#2$ \Downto $-\infty$ \Step $#3$  \While $#4$ \Do}}
%\newcommand{\ForFromTo}[3]{{\For $#1\in #2..#3$ \Do}}
%\newcommand{\ForFromToDown}[3]{{\For $#1\in #2..#3$ \textbf{downwards} \Do}}
%\newcommand{\ForFromWhile}[3]{{\For $#1\in #2..$ \While $#3$ \Do}}
%\newcommand{\ForFromDownWhile}[3]{{\For $#1\in #2..$ \textbf{downwards} \While $#3$ \Do}}
%\newcommand{\ForFromToStep}[4]{{\For $#1\in #2..#3$ \Step $#4$ \Do}}
%\newcommand{\ForFromToDownStep}[4]{{\For $#1\in #2..#3$ \textbf{downwards} \Step $#4$  \Do}}
%\newcommand{\ForFromWhileStep}[4]{{\For $#1\in #2..$ \While $#3$ \Step $#4$  \Do}}
%\newcommand{\ForFromDownWhileStep}[4]{{\For $#1\in #2..$ \textbf{downwards} \While $#3$ \Step $#4$  \Do}}
\newcommand{\End}       {\textbf{end\ }}
\newcommand{\Endfor}       {\textbf{endfor\ }}
\newcommand{\Rem}[1]   {\textbf{(*~}\textrm{#1}\textbf{~*)}}
% rechtsbuendiger Kommentar
%\newcommand{\RRem}[1]   {\`{$\mathbf{(*}$~ }\textrm{#1}{~$\mathbf{*)}$}}
\newcommand{\RRem}[1]   {\`\textbf{--\hspace{0.5mm}--~}\textrm{#1}}
\newcommand{\RRemNL}[1]   {\`\textbf{(*~ }\textrm{#1}\textbf{~*)}%
{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}
\newcommand{\Access}{\!\rightarrow\!}

\newcommand{\At}[1]{\left\langle#1\right\rangle}
\newcommand{\NL}{\`{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}

% Parallelverarbeitungspseudocode
\newcommand{\iProc}{i_\mathrm{PE}}

% Parameter 1=pos, 2=xsize, 3=filename, 4=llabel, 4=caption
\newcommand{\dissepslong}[5]{\begin{figure}[#1]\begin{center}%
\epsfxsize#2\leavevmode\epsfbox{#3.eps}%
\end{center}\caption{\llabel{#4}#5}\end{figure}}

\newcommand{\dissepspos}[4]{\dissepslong{#1}{#2}{\labelprefix/#3}{#3}{#4}}
\newcommand{\disseps}[3]{\dissepspos{htb}{#1}{#2}{#3}}

% Beweise
\newdimen\endofsize\endofsize=0.5em
\def\endofbeweis{~\quad\hglue\hsize minus\hsize
                 \hbox{\vrule height \endofsize width
\endofsize}\par}
% gibt es in amsmath schon
%\newenvironment{proof}{\textbf{Proof:} }{\endofbeweis}
% \newcommand{\platsch}{\hglue\hsize minus\hsize}

% Definitions of Sebastian Egner
% ==============================

% \invisible{<text>} produces an mbox without of <text>.
\newcommand{\invisible}[1]{\setbox0=\hbox{#1}%
\makebox[\wd0]{\raisebox{0pt}[\ht0][\dp0]{}}}

% \Z gives the nice `Z' to denote the integers
%\newcommand{\Z}[0]{%
%\textrm{\sf\setbox0=\hbox{Z}Z\makebox[-\wd0]{}\,Z}}
\newcommand{\Z}[0]{{\mathbb{Z}}}

% \Q gives the nice `Q' to denote the rationals
%\newcommand{\Q}[0]{%
%\textrm{\sf\setbox0=\hbox{Q}Q\makebox[-\wd0]{}\,I\,\,}}
%\newcommand{\Q}[0]{{\mathbb{Q}}}

% \R gives the nice `R' to denote reals
%\newcommand{\R}[0]{\mbox{$\rm\sf I\!R$}}
\newcommand{\R}[0]{{\mathbb{R}}}

% \C gives the nice `C' to denote complex numbers
%\newcommand{\C}[0]{\mbox{$\rm\sf I\!\!\!C$}}
\providecommand{\C}[0]{{\mathbb{C}}}
\renewcommand{\C}[0]{{\mathbb{C}}}

% \F gives the nice `F' to denote a generic field
\newcommand{\F}[0]{\textrm\textsf{F}}

% \GL gives the nice `GL' to denote invertible matrices
\newcommand{\GL}[0]{\textrm\textsf{GL}}

% \GF gives the nice 'F' to denote finite fields
%\newcommand{\GF}[1]{\mbox{$\rm\sf I\!R_{#1}$}}
\newcommand{\GF}[1]{{\mathbb{F}_{#1}}}

% bigsqcap_{#1} (has been forgotten in TeX)
\newcommand{\bigsqcap}[1]{
  \hspace{-1.0em}\raisebox{-1.0ex}{
    \renewcommand{\arraystretch}{0.5}
    $\begin{array}{c}
      \mbox{\LARGE$\sqcap$}  \\
      \mbox{\scriptsize$#1$}
    \end{array}$}\!\!}

% combinations n choose k
\newcommand{\combinations}[2]{%
{\renewcommand{\arraystretch}{0.8}%
 \setlength{\arraycolsep}{0.2em}%
 \left( \begin{array}{c} {#1} \\ {#2} \end{array} \right)}}

% \smallexpr{<expr>} puts <expr> in \footnotesize
\newcommand{\smallexpr}[1]{\mbox{\footnotesize$#1$}}

% \smallsmallexpr{<expr>} puts <expr> in \scriptsize
\newcommand{\smallsmallexpr}[1]{\mbox{\scriptsize$#1$}}

% a prominent problem
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}

% \begin{definition} .. \end{definition} gives a def.
%\newtheorem{definition}[theorem]{Definition}

%\newtheorem{corollary}[theorem]{Corollary}


% \begin{algorithm} .. \end{algorithm} gives an algorithm
%\newenvironment{algorithm}%
%{\par\vspace{1.0ex}\noindent\textbf{Algorithm}\ }%
%{\par\vspace{-1.5ex}\noindent}

% \begin{proof} .. \end{proof} gives a proof
%\newenvironment{proof}%
%{\vspace{0.5ex}\noindent\textbf{Proof:}\ }%
%{\par\vspace{0.5ex}\noindent}%

% q.e.d. sign
%\newcommand{\qed}[0]{\hfill\rule{1ex}{1ex}}
%\newcommand{\qed}[0]{~\mbox{$\triangleleft$}}
%\newcommand{\qed}[0]{\hfill\mbox{$\Box$}}


\usepackage{graphicx}

\newcommand*\openquote{\makebox(25,-22){\scalebox{5}{``}}}
\newcommand*\closequote{\makebox(25,-22){\scalebox{5}{''}}}

